A Terabit Hybrid FPGA-ASIC Platform for Switch Virtualization

The roll-out of technologies like 5G and the need for multi-terabit bandwidth in backbone networks requires networking companies to make significant investments to keep up with growing service demands. For lower capital expenditure and faster time-to-market, companies can resort to anything-as-a-service providers to lease virtual resources. Nevertheless, existing virtualization technologies are still lagging behind next-generation networks' requirements. This paper breaks the terabit barrier by introducing a hybrid FPGA-ASIC architecture to virtualize programmable forwarding planes. In contrast to existing solutions, our architecture involves an ASIC that multiplexes network flows between programmable virtual switches running in an FPGA capable of full and partial reconfiguration, enabling virtual switch hot-swapping. Our evaluation shows the feasibility of a switch virtualization architecture capable of achieving a combined throughput of 3.2 Tbps by having up to 26 virtual switch instances in parallel with low resource occupation overhead.

==> acronyms.tex <==
\newacronym{gpu}{GPU}{Graphics Processing Unit}
\newacronym{cnn}{CNN}{Convolutional Neural Network}
\newacronym{flop}{FLOP}{FLoating-point Operations Per Second}
\newacronym{asild}{ASIL-D}{Automotive Safety Integrity Level D}
\newacronym{sdc}{SDC}{Single Data Corruption}
\newacronym{secded}{SECDED}{Single Error Correction Double Error Detection}
\newacronym{dmr}{DMR}{Double Modular Redundancy}
\newacronym{fit}{FIT}{Failure In Time}
\newacronym{kvf}{KVF}{Kernel Vulnerability Factor}
\newacronym{adas}{ADAS}{Advanced Driver Assistance Systems}
\newacronym{hog}{HOG}{Histogram of Oriented Gradients}
\newacronym{yolo}{YOLO}{You Only Look Once}
\newacronym{ecc}{ECC}{Error Correction Code}
\newacronym{hpc}{HPC}{High Performance Computing}
\newacronym{svm}{SVM}{Support Vector Machine}
\newacronym[\glslongpluralkey={Bounding Boxes}]{bb}{BB}{Bounding Box}
\newacronym{dnn}{DNN}{Deep Neural Network}
\newacronym{lvf}{LVF}{Layer Vulnerability Factor}
\newacronym{relu}{ReLU}{Rectified Linear Units}
\newacronym{ann}{ANN}{Artificial Neural Network}
\newacronym{pvf}{PVF}{Program Vulnerability Factor}
\newacronym{avf}{AVF}{Architecture Vulnerability Factor}
\newacronym{tmr}{TMR}{Tiple Modular Redundancy}
\newacronym{rf}{RF}{Register File}
\newacronym{inst}{INST}{Instruction}


==> recycle-bin.tex <==

    % DSLs
    The concept of programmable forwarding planes has seen a renewed interest by industry and academia with the advent of domain-specific languages (DSL) like POF~\cite{Song:2013:PFU:2491185.2491190}, P4~\cite{Bosshart:2014:P4}, and Lyra~\cite{Lyra}. These languages unleashed innovation in the data plane~\cite{daCostaCordeiro2017}, helping break further the ``network ossification'', and reshaped its research agenda to include aspects from switch program composition to verification and switch debugging.
    % Falar mais um pouco de como DSLs podem impactar "After 5G and Multi-Gigabit Communications"
    
    % Virtualization
    Virtualization is nice.

    % Resource sharing
    Resource sharing through virtualization has become commonplace in modern public and private clouds, powering virtual abstractions for servers \cite{multi-tenant-networks-nsdi-2014}, network functions \cite{clickos-nsdi-2014,hwang2015netvm,clicknp,yi2018comprehensive}, forwarding devices \cite{routebricks,sherwood2009flowvisor,openvswitch-nsdi15,pisces-sigcomm-16,picnic-sigcomm2019}, and even entire control planes \cite{covisor-nsdi2015,blenk2015survey,afolabi2018network} running atop a shared infrastructure. These virtual abstractions are highly convenient, as they enable efficient resource usage for network providers and resource isolation for network tenants.
    % Fazer o link com 5G e afins
    
    % After 5G and Multi-Gigabit Communications
    5G is a great example, but applies to future technologies.
    
    % Related works and examples
    SUME towards 100G: \cite{SUME_micro}.
    Trident: \cite{TRIDENT}.
    Tofino: \cite{TOFINO}.
    Silicon One: \cite{SILICON_ONE}.
    
    % Proposal
    We propose a hybrid FPGA-ASIC platform implementation that combines the FPGA advantages of reconfigurability and flexibility with ASIC's increased clock frequencies for improved data throughput.
    % contribuiton
    To the best of our knowledge, this is the first work in the literature to break the terabit mark while offering switch virtualization, hot-swap reprogrammability, and backend scalability.
    

